Automated Evolutionary Approach for the Design of Composite Machine Learning Pipelines

The effectiveness of the machine learning methods for real-world tasks depends on the proper structure of the modeling pipeline. The proposed approach is aimed to automate the design of composite machine learning pipelines, which is equivalent to computation workflows that consist of models and data operations. The approach combines key ideas of both automated machine learning and workflow management systems. It designs the pipelines with a customizable graph-based structure, analyzes the obtained results, and reproduces them. The evolutionary approach is used for the flexible identification of pipeline structure. The additional algorithms for sensitivity analysis, atomization, and hyperparameter tuning are implemented to improve the effectiveness of the approach. Also, the software implementation on this approach is presented as an open-source framework. The set of experiments is conducted for the different datasets and tasks (classification, regression, time series forecasting). The obtained results confirm the correctness and effectiveness of the proposed approach in the comparison with the state-of-the-art competitors and baseline solutions.

==> add.tex <==
% Auto-sklearn is a plugin linked to the scikit-learn library. To use this module, users need to specify how the provided data will be scored, as well as bounds for scoring each machine learning pipeline and hyperparameters for the join strategy (which replaces the model selection process inside Auto-sklearn). This framework shows good results for small and medium-size datasets, but performance is poor when working with large datasets.

% Next, we will consider the frameworks aimed at automated selection of the neural network architecture.
% TPOT (Tree-based Pipeline Optimization Tool) is a tree-based machine learning pipeline optimization tool that uses genetic algorithms as an optimizer. This framework is based on scikit-learn.

% MLBox is a library from the Python language that provides the following functionality: fast data reading and preprocessing operations (cleaning, formatting), optimization of model hyperparameters, creation of classification and regression models with the possibility of interpretation.

% H2O is an open source machine learning platform. It supports programming languages Python and R \citep{H2OAutoML20}. H2O also allows for preprocessing data, applying many commonly used algorithms for machine and statistical learning. In the process of work, two ensembles of models are used, which are trained using meta-learning. The search is carried out on a grid and ends when the maximum number of models or time limit is reached. In addition, automatic visualization and interpretation is performed.

Also, it`s worth mentioning the development toolkit from Google – AutoML Tables. This tool allows you to very quickly design and deploy modern machine learning models in automatic mode. AutoML Tables allows to process structured data in the cloud.

The study \citep{zoller2021benchmark} provides an overview of various AutoML methods and a comparison of the effectiveness of frameworks and approaches, which were mentioned before (TPOT, Hpsklearn, Auto-Sklearn, Random Search, H2O) on 137 datasets. Summing up the results of the study, the authors state that modern frameworks are still unable to produce a model that could surpass the models created by experts. However, the advantages of using frameworks include the ease of creating effective machine learning pipelines.


==> add2.tex <==
% \begin{algorithm}
% \SetKwData{adaptedCompositeModel}{adaptedCompositeModel}
%  \SetKwData{compositeModel}{compositeModel}
%   \SetKwData{initialCompositeModel}{initialCompositeModel}
%   \SetKwData{atomizedModel}{atomizedModel}

%  \SetKwData{candidateCompositeModel}{candidateCompositeModel}
%  \SetKwData{quality}{quality}
%  \SetKwData{bestQuality}{bestQuality}
%  \SetKwData{maxTime}{maxTime}
%  \SetKwData{retrainData}{retrainData}
%  \SetKwData{validationData}{validationData}
%   \SetKwData{trainData}{trainData}
%   \SetKwData{testData}{testData}
%   \SetKwData{popSize}{popSize}
%     \SetKwData{fitness}{fitness}
%   \SetKwData{pop}{pop}
%  \SetKwFunction{Evolution}{Evolution}
%   \SetKwFunction{Atomize}{Atomize}

%  \SetKwFunction{Fit}{Fit}
%   \SetKwFunction{Split}{Split}
%     \SetKwFunction{Repeat}{Repeat}
%   \SetKwFunction{ConvergenceCriterion}{ConvergenceCriterion}
%     \SetKwFunction{TimeLimit}{TimeLimit}
%     \SetKwFunction{CalcMetric}{CalcMetric}

%  \SetKwFunction{EvaluateQuality}{EvaluateQuality}
%  \SetKwFunction{Best}{Best}
%  \SetKwFunction{FineTuneParams}{FineTuneParams}
%  \SetKwFunction{Assert}{Assert}
%  \KwData{\maxTime, \retrainData, \initialCompositeModel}
%   \KwResult{\adaptedCompositeModel}
  
%  \atomizedModel $\leftarrow$ \Atomize(\initialCompositeModel)
 
%  \pop  $\leftarrow$ \Repeat{\atomizedModel, \popSize} \\
%  \trainData, \testData = \Split{\retrainData}
 
%  \While {not ConvergenceCriterion() or TimeLimit(\maxTime)}  {
%     \For {\compositeModel in \pop} {
%         \compositeModel.\fitness $\leftarrow$ \CalcMetric{\compositeModel,\trainData, \testData}
%      }
     
%      \pop = \Evolution{\pop}
     
%  }

% \adaptedCompositeModel = \Best{\pop}

% \adaptedCompositeModel = \FineTuneParams{\adaptedCompositeModel}


% \Assert \CalcMetric{\adaptedCompositeModel, \retrainData, \validationData} $>$ \CalcMetric{\initialCompositeModel, \retrainData, \validationData}

%  \caption{The pseudocode of the composite models atomization and additional learning}
%  \label{alg_hyperopt}
% \end{algorithm}
